The Model Openness Framework: Promoting Completeness and Openness for Reproducibility, Transparency, and Usability in Artificial Intelligence

Generative artificial intelligence (AI) offers numerous opportunities for research and innovation, but its commercialization has raised concerns about the transparency and safety of frontier AI models. Most models lack the necessary components for full understanding, auditing, and reproducibility, and some model producers use restrictive licenses whilst claiming that their models are "open source". To address these concerns, we introduce the Model Openness Framework (MOF), a three-tiered ranked classification system that rates machine learning models based on their completeness and openness, following open science principles. For each MOF class, we specify code, data, and documentation components of the model development lifecycle that must be released and under which open licenses. In addition, the Model Openness Tool (MOT) provides a user-friendly reference implementation to evaluate the openness and completeness of models against the MOF classification system. Together, the MOF and MOT provide timely practical guidance for (i) model producers to enhance the openness and completeness of their publicly-released models, and (ii) model consumers to identify open models and their constituent components that can be permissively used, studied, modified, and redistributed. Through the MOF, we seek to establish completeness and openness as core tenets of responsible AI research and development, and to promote best practices in the burgeoning open AI ecosystem.

==> Archived-text.tex <==
\subsection{Open Source AI}
\label{sec:opensource-ai}
Open source AI technology enables anyone to reuse and improve the  technology. “Open source AI technology” include the model architecture, model weights and parameters, source code, configuration files, and information about the data used to train the system that are collectively published under licenses allowing any recipient to, without restriction, to use, study, distribute, sell, copy, create derivative works of, and make modifications to, the licensed artifacts or modified versions thereof.

\subsection{Open Science AI}
\label{sec:openscience-ai}
Open science AI technology enables anyone to reuse and improve an AI technology, while providing additional transparency and reproducibility. “Open science AI technology” is an open source AI technology that additionally include licenses to all source code, training data, configuration files, research, and documentation required to reproduce a similar AI technology without restriction.
